Learning Clothing and Pose Invariant 3D Shape Representation for Long-Term Person Re-Identification

Long-Term Person Re-Identification (LT-ReID) has become increasingly crucial in computer vision and biometrics. In this work, we aim to extend LT-ReID beyond pedestrian recognition to include a wider range of real-world human activities while still accounting for cloth-changing scenarios over large time gaps. This setting poses additional challenges due to the geometric misalignment and appearance ambiguity caused by the diversity of human pose and clothing. To address these challenges, we propose a new approach 3DInvarReID for (i) disentangling identity from non-identity components (pose, clothing shape, and texture) of 3D clothed humans, and (ii) reconstructing accurate 3D clothed body shapes and learning discriminative features of naked body shapes for person ReID in a joint manner. To better evaluate our study of LT-ReID, we collect a real-world dataset called CCDA, which contains a wide variety of human activities and clothing changes. Experimentally, we show the superior performance of our approach for person ReID.

==> fig/sec_5_conclusion.tex <==


\section{Conclusions}\label{sec:con}

This paper tackles the challenging setting of long-term person ReID, which allows a wider range of real-world human activities and accounts for cloth-changing scenarios.
%
To address this problem, we present a joint two-layer implicit representation to model textured $3$D clothed humans together with a discriminative fitting module, enabling us to disentangle identity and non-identity features for real-world images. 
%
We collect a new LT-ReID dataset, CCDA, with diverse human activities and clothing changes, facilitating future research on real-world scenarios.
%
Experimental results demonstrate the effectiveness of our method in disentangling identity and non-identity features in $3$D clothed body shapes, thereby contributing to LT-ReID.



\Paragraph{Limitations \& Potential Negative Impacts Impacts}
Our work tackles the challenge of disentangling clothing and body shape in $3$D shape representation. The clothing reconstruction task remains challenging as evidenced by the visual quality of the published models and our models. Our results show that the task of body-clothing disentanglement brings benefit in the recognition task, a finding which opens new possibilities to multi-task learning across $2$D-$3$D modalities. Like most person ReID
methods, one potential negative impact of our approach is that it could be used for unethical surveillance and invasion of privacy.

\Paragraph{Acknowledgments} This research is based upon work supported by the Office of the Director of National Intelligence (ODNI), Intelligence Advanced Research Projects Activity (IARPA), via 2022-21102100004. The views and conclusions contained herein are those of
the authors and should not be interpreted as necessarily representing the official policies, either expressed or implied, of ODNI, IARPA, or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for governmental purposes notwithstanding any copyright annotation therein.

